The connection between mass, environment and slow rotation in simulated galaxies

Recent observations from integral field spectroscopy (IFS) indicate that the fraction of galaxies that are slow rotators, $F_{\rm SR}$, depends primarily on stellar mass, with no significant dependence on environment. We investigate these trends and the formation paths of slow rotators (SRs) using the EAGLE and Hydrangea hydro-dynamical simulations. EAGLE consists of several cosmological boxes of volumes up to $(100\,\rm Mpc)^3$, while Hydrangea consists of $24$ cosmological simulations of galaxy clusters and their environment. Together they provide a statistically significant sample in the stellar mass range $10^{9.5}\,\rm M_{\odot}-10^{12.3}\,\rm M_{\odot}$, of $16,358$ galaxies. We construct IFS-like cubes and measure stellar spin parameters, $\lambda_{\rm R}$, and ellipticities, allowing us to classify galaxies into slow/fast rotators as in observations. The simulations display a primary dependence of $F_{\rm SR}$ on stellar mass, with a weak dependence on environment. At fixed stellar mass, satellite galaxies are more likely to be SRs than centrals. $F_{\rm SR}$ shows a dependence on halo mass at fixed stellar mass for central galaxies, while no such trend is seen for satellites. We find that $\approx 70$% of SRs at $z=0$ have experienced at least one merger with mass ratio $\ge 0.1$, with dry mergers being at least twice more common than wet mergers. Individual dry mergers tend to decrease $\lambda_{\rm R}$, while wet mergers mostly increase it. However, $30$% of SRs at $z=0$ have not experienced mergers, and those inhabit halos with median spins twice smaller than the halos hosting the rest of the SRs. Thus, although the formation paths of SRs can be varied, dry mergers and/or halos with small spins dominate.

==> Makefile <==
SHELL=/bin/bash
NOMBRE=$(shell grep -H \\documentclass *.tex | cut -d: -f1 | cut -d. -f1)

ifeq ($(strip $(wildcard $(NOMBRE).bib) ),)
HAVE_BIB=no
else
HAVE_BIB=yes
endif



DEPENDENCIES=$(NOMBRE).tex

ifeq '$(HAVE_BIB)' 'yes'
DEPENDENCIES+= $(NOMBRE).bib
endif

HAVE_BIB=yes

all: $(NOMBRE).pdf

$(NOMBRE).pdf: $(DEPENDENCIES)
	@echo "   Making dvi for first time..."
	@latex -halt-on-error $(NOMBRE).tex &> .my_log || (cat .my_log && rm .my_log && exit 1)
	@rm .my_log
	@if [[ "${HAVE_BIB}" == "yes" ]]; then \
	echo "   Compiling references..." && \
	(bibtex $(NOMBRE) &> .my_log || (cat .my_log && rm .my_log && exit 1)) && \
	rm .my_log && \
	echo "   Re-making dvi including bibliography..." && \
	latex $(NOMBRE).tex &> /dev/null; \
	fi
	@echo "   Re-making dvi for satisfying references..."
	@latex $(NOMBRE).tex &> /dev/null
	@echo "   Generating final pdf..."
	@dvipdf $(NOMBRE).dvi &> /dev/null

clean:
	-rm -f $(NOMBRE).{aux,toc,log,tmp,dvi,idx,ilg,ind,bbl,blg,out} .my_log

distclean: clean
	-rm -f $(NOMBRE).pdf

k: $(NOMBRE).pdf
	@echo "   Opening $(NOMBRE).pdf with okular..."
	@okular $(NOMBRE).pdf &> /dev/null &

x: $(NOMBRE).pdf
	@echo "   Opening $(NOMBRE).pdf with xpdf..."
	@xpdf $(NOMBRE).pdf &> /dev/null &

